An Innovative Information Theory-based Approach to Tackle and Enhance The Transparency in Phishing Detection

Phishing attacks have become a serious and challenging issue for detection, explanation, and defense. Despite more than a decade of research on phishing, encompassing both technical and non-technical remedies, phishing continues to be a serious problem. Nowadays, AI-based phishing detection stands out as one of the most effective solutions for defending against phishing attacks by providing vulnerability (i.e., phishing or benign) predictions for the data. However, it lacks explainability in terms of providing comprehensive interpretations for the predictions, such as identifying the specific information that causes the data to be classified as phishing. To this end, we propose an innovative deep learning-based approach for email (the most common phishing way) phishing attack localization. Our method can not only predict the vulnerability of the email data but also automatically learn and figure out the most important and phishing-relevant information (i.e., sentences) in the phishing email data where the selected information indicates useful and concise explanations for the vulnerability. The rigorous experiments on seven real-world diverse email datasets show the effectiveness and advancement of our proposed method in selecting crucial information, offering concise explanations (by successfully figuring out the most important and phishing-relevant information) for the vulnerability of the phishing email data. Particularly, our method achieves a significantly higher performance, ranging from approximately 1.5% to 3.5%, compared to state-of-the-art baselines, as measured by the combined average performance of two main metrics Label-Accuracy and Cognitive-True-Positive.

==> sections/discussion.tex <==
\section{Discussion}\label{sec:discussion}
\subsection{Threats to Validity}
\label{sec:threats}

\paragraph{Construct Validity}
Key construct validity threats are if our assessments of the proposed method and baselines demonstrate the ability for phishing attack localization. In our paper, we study an important problem of phishing attack localization where we not only aim to automatically learn and figure out the important phishing-relevant information (e.g., sentences) in each phishing email but also can detect the vulnerability $Y$ (i.e., phishing or benign) of the corresponding email based on the crucial selected information. The selected phishing-relevant information (e.g., sentences) helps provide comprehensive explanations about the vulnerability of the phishing email data. To evaluate the performance of our method and baselines, we introduce three main measures including Label-Accuracy, Cognitive-True-Positive, and SAC.

\paragraph{Internal Validity}
Key internal validity threats are relevant to the choice of hyper-parameter settings (i.e., optimizer, learning rate, number of layers in deep neural networks, etc.). It is worth noting that finding a set of optimal hyperparameter settings of deep neural networks is expensive due to a large number of trainable parameters. To train our method, we only use the common and default values of hyper-parameters such as using Adam optimizer and the learning rate equals $10^{-3}$. We also report the hyperparameter settings in the released reproducible source code to support future replication studies.

\paragraph{External Validity}
Key external validity threats include whether our proposed \ourapp~ method can generalize well to different phishing vulnerabilities and other different types of phishing email datasets. We mitigated this problem by conducting our experiments on seven public phishing email datasets including IWSPA-AP, Nazario Phishing Corpus, Miller Smiles Phishing Email, Phish Bowl Cornell University, Fraud emails, Cambridge, and Enron Emails.
